Total progeny in killed branching random walk

We consider a branching random walk for which the maximum position of a particle in the n'th generation, M_n, has zero speed on the linear scale: M_n/n --> 0 as n --> infinity. We further remove ("kill") any particle whose displacement is negative, together with its entire descendence. The size $Z$ of the set of un-killed particles is almost surely finite. In this paper, we confirm a conjecture of Aldous that Exp[Z] < infinity while Exp[Z log Z]=infinity. The proofs rely on precise large deviations estimates and ballot theorem-style results for the sample paths of random walks.

==> mean_progeny.tex <==
%!TEX root = killedbrw.tex

\begin{lem}Let $Z$ be the total progeny of a critical killed branching random walk. Then, $\e Z <\infty$.
\end{lem}  
\begin{proof}Let $\mathscr L_n$ denote the set of individuals in generation $n$. Then, we have
\begin{eqnarray*}
\E{Z} = \sum_{n\ge 0} \E{\#\{u\in \mathscr L_n: u \in T\}}&=&\sum_{n\ge 0} \E{B}^n \cdot \p{S_i\ge 0, 0\le i\le n}\\   
&=&\sum_{n\ge 0} \E{B}^n \cdot \sum_{k\ge 0} \p{S_i\ge 0, 1\le i\le n; S_n=k}.                                
\end{eqnarray*}  
Splitting the sum above at $k=\log^2 n$, and using Theorems~\ref{thm:} and~\ref{thm:}, we obtain for $n$ large enough
\begin{eqnarray*}
\E{\#\{u\in \mathscr L_n: u \in T\}}         
&\le&\E{B}^n \cdot \sum_{k=0}^{\lfloor\log^2 n\rfloor}\p{S_i\ge 0, 0\le i\le n; S_n=k} + \E{B}^n \cdot \p{S_n \ge \log^2 n}\\
&\le& \sum_{k=0}^{\lfloor\log^2 n\rfloor}\Cprob{S_i\ge 0, 0\le i\le n}{S_n=k} \cdot \frac{C_1 e^{-t k}}{\sqrt n}+ e^{-t \log^2 n}\\
&\le & C_2 \sum_{k=0}^{\lfloor \log^2 n\rfloor} \frac{k e^{-t k}}{n^{3/2}} + e^{-t \log^2 n}\le C_3 n^{-3/2},
\end{eqnarray*}
for some constants $C_1,C_2, C_3$. It follows immediately that $\E{Z}<\infty$.
\end{proof}
